Twistor Construction of Higher-Dimensional Black Holes - Part II: Examples

We apply the twistor construction for higher-dimensional black holes to known examples in five space-time dimensions. First the patching matrices are calculated from the explicit metric for these examples. Then an ansatz is proposed for obtaining the patching matrix instead from the data of rod structure and angular momenta. The ansatz is tested on examples with up to three nuts, and these are shown to give flat space, the Myers-Perry solution and the black ring, as expected. Rules for the transition between different adaptations of the patching matrix and for the elimination of conical singularities are developed and seen to work.

==> headings.tex <==
%% heading style %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%section%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}%
                                   {2.3ex \@plus.2ex}%
                                   {\normalfont\large\bfseries}}
\makeatother

%subsection%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\subsection{\@ifstar\unnumberedsubsection\numberedsubsection}
\def\numberedsubsection{\@ifnextchar[%]
  \numberedsubsectionwithtwoarguments\numberedsubsectionwithoneargument}
\def\unnumberedsubsection{\@ifnextchar[%]
  \unnumberedsubsectionwithtwoarguments\unnumberedsubsectionwithoneargument}
\def\numberedsubsectionwithoneargument#1{\numberedsubsectionwithtwoarguments[#1]{#1}}
\def\unnumberedsubsectionwithoneargument#1{\unnumberedsubsectionwithtwoarguments[#1]{#1}}
\def\numberedsubsectionwithtwoarguments[#1]#2{%
  \ifhmode\par\fi
  \removelastskip
  \vskip 3ex\goodbreak
  \refstepcounter{subsection}%
  \noindent
  \leavevmode
  \begingroup
  \bfseries \indent
  \thesubsection\ 
  #2. 
  \endgroup
  \addcontentsline{toc}{subsection}{%
    \protect\numberline{\thesubsection}%
    #1}%
  }
\def\unnumberedsubsectionwithtwoarguments[#1]#2{%
  \ifhmode\par\fi
  \removelastskip
  \vskip 3ex\goodbreak
%  \refstepcounter{section}%
  \noindent
  \leavevmode
  \begingroup
  \bfseries \indent
%  \thesubsection\ 
  #2.
  \endgroup
%  \addcontentsline{toc}{subsection}{%
%    \protect\numberline{\thesection}%
%    #1}%
  }
\makeatother


%subsubsection%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\def\subsubsection{\@ifstar\unnumberedsubsubsection\numberedsubsubsection}
\def\numberedsubsubsection{\@ifnextchar[%]
  \numberedsubsubsectionwithtwoarguments\numberedsubsubsectionwithoneargument}
\def\unnumberedsubsubsection{\@ifnextchar[%]
  \unnumberedsubsubsectionwithtwoarguments\unnumberedsubsubsectionwithoneargument}
\def\numberedsubsubsectionwithoneargument#1{\numberedsubsubsectionwithtwoarguments[#1]{#1}}
\def\unnumberedsubsubsectionwithoneargument#1{\unnumberedsubsubsectionwithtwoarguments[#1]{#1}}
\def\numberedsubsubsectionwithtwoarguments[#1]#2{%
  \ifhmode\par\fi
  \removelastskip
  \vskip 2ex\goodbreak
  \refstepcounter{subsubsection}%
  \noindent
  \leavevmode
  \begingroup
  \itshape \indent
  \thesubsubsection\ 
  #2.
  \endgroup
  \addcontentsline{toc}{subsubsection}{%
    \protect\numberline{\thesubsubsection}%
    #1}%
  }
\def\unnumberedsubsubsectionwithtwoarguments[#1]#2{%
  \ifhmode\par\fi
  \removelastskip
  \vskip 2ex\goodbreak
%  \refstepcounter{section}%
  \noindent
  \leavevmode
  \begingroup
  \itshape \indent
%  \thesubsubsection\ 
  #2.  
  \endgroup
%  \addcontentsline{toc}{subsubsection}{%
%    \protect\numberline{\thesubsubsection}%
%    #1}%
  }
\makeatother

%% ToC style %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\contentsnamefont{\large\bfseries}

\newcommand{\mycftdotsep}{5.5}
\newcommand{\mycftdotfill}[1]{%
  \leaders\hbox{$\mkern #1 mu\hbox{.}\mkern #1 mu$}\hfill}
  
%% defines whether the sections are in bold or note
%% \bfseries = in bold, \mdseries = not bold
\newcommand{\Myseries}{\mdseries}

\makeatletter
\def\l@part{\@tocline{-1}{3pt plus1pt}{1pc}{}{\bfseries}}  
\def\appendixname{} 
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\@M
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
    \rightskip\@pnumwidth plus4em \parfillskip-\@pnumwidth
    #5\leavevmode\hskip-\@tempdima #6\nobreak\relax
    \ifnum#1<1\hfill\else \mycftdotfill{\mycftdotsep} 
		\fi\hbox  to\@pnumwidth{\ifnum#1<2\@tocpagenumBF{#7\hspace{1.2em}}\else\@tocpagenum{#7\hspace{1.2em}}\fi}\par
    \nobreak
    \endgroup
  \fi}
  \def\@tocpagenumBF#1{\hss{\Myseries #1}}
  \renewcommand{\tocsection}[3]{%
    \indentlabel{\@ifnotempty{#2}{\Myseries\ignorespaces#1 \makebox[1.0em][l]{#2.} }}\Myseries #3}
  \def\l@subsection{\@tocline{2}{0pt}{2.3pc}{5pc}{}}
  \renewcommand{\tocsubsection}[3]{%
    \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 \makebox[1.7em][l]{#2.} }}\mdseries #3}
  \def\l@subsubsection{\@tocline{3}{0pt}{4pc}{7pc}{}} %%%  2.3pc or 4.0pc
  \renewcommand{\tocsubsubsection}[3]{%
    \indentlabel{\@ifnotempty{#2}{\ignorespaces#1 \makebox[2.5em][l]{#2.} }}\mdseries #3}
\makeatother

%%% citestyle %%%%%%%%%%%%%%%%%%%%
\def\citeform#1{{\mdseries#1}}
